Rendering of Eyes for Eye-Shape Registration and Gaze Estimation

Images of the eye are key in several computer vision problems, such as shape registration and gaze estimation. Recent large-scale supervised methods for these problems require time-consuming data collection and manual annotation, which can be unreliable. We propose synthesizing perfectly labelled photo-realistic training data in a fraction of the time. We used computer graphics techniques to build a collection of dynamic eye-region models from head scan geometry. These were randomly posed to synthesize close-up eye images for a wide range of head poses, gaze directions, and illumination conditions. We used our model's controllability to verify the importance of realistic illumination and shape variations in eye-region training data. Finally, we demonstrate the benefits of our synthesized training data (SynthesEyes) by out-performing state-of-the-art methods for eye-shape registration as well as cross-dataset appearance-based gaze estimation in the wild.

==> figs/fig_example_fits_MPII.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_0.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_55.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_160.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_12.png}
    \par \vspace{0.1em}
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_35.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_145.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_171.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_113.png}
    \par \vspace{0.1em}
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_179.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_42.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_63.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/ldmks_examples/idx_96.png}
    %
    \caption{The top two rows illustrate successful eye-shape registration on MPIIGaze. The bottom row illustrates failure cases.}
    \label{fig:clnf_examples}
\end{figure}


==> figs/fig_example_fits_wild.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_550.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_560.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_799.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_721.png}
    \par \vspace{0.1em}
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_1013.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_1002.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_765.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_508.png}
    \par \vspace{0.1em}
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_934.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_875.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_913.png}\hfill
    \includegraphics[width=0.244\columnwidth]{figs/wild_ldmks_examples/idx_953.png}
    %
    \caption{The top two rows illustrate successful eye-shape registration on 300-W. The bottom row illustrates failure cases, including un-modelled occlusions and eyelid poses.}
    \label{fig:example_fits_wild}
\end{figure}
